Modulation of DNA rheology by a transcription factor that forms aging microgels

Proteins and nucleic acids form non-Newtonian liquids with complex rheological properties that contribute to their function in vivo. Here we investigate the rheology of the transcription factor NANOG, a key protein in sustaining embryonic stem cell self-renewal. We discover that at high concentrations NANOG forms macroscopic aging gels through its intrinsically disordered tryptophan-rich domain. By combining molecular dynamics simulations, mass photometry and Cryo-EM, we also discover that NANOG forms self-limiting micelle-like clusters which expose their DNA-binding domains. In dense solutions of DNA, NANOG micelle-like structures stabilize intermolecular entanglements and crosslinks, forming microgel-like structures. Our findings suggest that NANOG may contribute to regulate gene expression in a unconventional way: by restricting and stabilizing genome dynamics at key transcriptional sites through the formation of an aging microgel-like structure, potentially enabling mechanical memory in the gene network.

==> z1.tex <==



==> z2.tex <==


